An Interview Study on Third-Party Cyber Threat Hunting Processes in the U.S. Department of Homeland Security

Cybersecurity is a major challenge for large organizations. Traditional cybersecurity defense is reactive. Cybersecurity operations centers keep out adversaries and incident response teams clean up after break-ins. Recently a proactive stage has been introduced: Cyber Threat Hunting (TH) looks for potential compromises missed by other cyber defenses. TH is mandated for federal executive agencies and government contractors. As threat hunting is a new cybersecurity discipline, most TH teams operate without a defined process. The practices and challenges of TH have not yet been documented. To address this gap, this paper describes the first interview study of threat hunt practitioners. We obtained access and interviewed 11 threat hunters associated with the U.S. government's Department of Homeland Security. Hour-long interviews were conducted. We analyzed the transcripts with process and thematic coding.We describe the diversity among their processes, show that their processes differ from the TH processes reported in the literature, and unify our subjects' descriptions into a single TH process.We enumerate common TH challenges and solutions according to the subjects. The two most common challenges were difficulty in assessing a Threat Hunter's expertise, and developing and maintaining automation. We conclude with recommendations for TH teams (improve planning, focus on automation, and apprentice new members) and highlight directions for future work (finding a TH process that balances flexibility and formalism, and identifying assessments for TH team performance).

==> data/data.tex <==
% ============= MAVEN CENTRAL =================
\newcommand{\maven}{Maven Central\xspace}
\newcommand{\mavenPackages}{{\TODO{30}}\xspace}
\newcommand{\mavenOrganizations}{{\TODO{16}}\xspace}

\newcommand{\mavenReevaluateSelected }{{\TODO{10\%}}\xspace}


% ============= HUGGING FACE =================
\newcommand{\hf}{{Hugging Face}\xspace}
\newcommand{\hfPackages}{{\TODO{50}}\xspace}

% ============= DOCKER HUB =================
\newcommand{\docker}{{Docker Hub}\xspace}
\newcommand{\dockerPackages}{{\TODO{X}}\xspace}

% % ============= NPM =================
% \newcommand{\npm}{{NPM}\xspace}
% \newcommand{\npmPackages}{{\TODO{X}}\xspace}

% ============= PyPI =================
\newcommand{\pypi}{{PyPI}\xspace}
\newcommand{\pypiPackages}{{\TODO{X}}\xspace}




\newcommand{\registries}{{\maven, \hf, \docker, and \pypi}\xspace}

==> misc/typesetting.tex <==
% Pre-condition: Set the ifs: \ifDEBUG, \ifANONYMOUS, \ifSPACEHACK

%%%%%
% Standard packages
%%%%%


%\usepackage[compress]{cite} % numbered ordering of multiple citations, set to compress ranges
\usepackage{amsmath,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{booktabs} % For formal tables \toprule
\usepackage{xspace} % Put an \xspace within numeric macros
\usepackage[normalem]{ulem}
\usepackage{makecell}
\usepackage{tcolorbox}
\usepackage{enumitem}
\usepackage{siunitx}
\usepackage[vskip=1em,font=itshape,leftmargin=2em,rightmargin=2em]{quoting}
\usepackage{svg}
\usepackage{listings}
\usepackage{subfigure}
\usepackage{xcolor}
%\useunder{\uline}{\ul}{}
% \usepackage{filecontents,lipsum}
% \usepackage[noadjust]{cite}
%%%%%
% Comments and TODOs
%%%%%

\usepackage{soul}
\usepackage{hyperref}
\usepackage{cleveref}

\ifDEBUG
    % Floating comment boxes
    \newcommand{\JD}[1]{\textcolor{purple}{[Jamie: #1]}}
    \newcommand{\Kelechi}[1]{\textcolor{olive}{[Kelechi: #1]}}
    \newcommand{\TRS}[1]{\textcolor{teal}{[Taylor: #1]}}
    \newcommand{\AK}[1]{\textcolor{blue}{[Andy: #1]}}
    
    % Inline comments and WIP phrasing
    \newcommand{\TODO}[1]{\hl{#1}}
\else
    \newcommand{\JD}[1]{}
    \newcommand{\Kelechi}[1]{}
    \newcommand{\TRS}[1]{}
    \newcommand{\AK}[1]{}

    \newcommand{\TODO}[1]{#1}
\fi

%%%%%
% Paragraph-level labels
%%%%%

%%%%%
% Space hacking
%%%%%

% To reduce spacing after headings %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{titlesec}

% \usepackage[compact]{titlesec}
% \titleformat{\section}
%   {\normalfont\Large\bfseries}{\thesection}{1em}{\MakeUppercase}
%     % The bug in the new version 2.10.1 is not properly starting horizontal mode
%     % http://tex.stackexchange.com/questions/299969/titlesec-loss-of-section-numbering-with-the-new-update-2016-03-15
%     \usepackage{etoolbox}
%     \makeatletter
%     \patchcmd{\ttlh@hang}{\parindent\z@}{\parindent\z@\leavevmode}{}{}
%     \patchcmd{\ttlh@hang}{\noindent}{}{}{}
%     \makeatother

% Make a \paragraph that is inline and emphasized
\newcommand{\myparagraph}[1]{\vspace{0.08cm}\noindent\hspace{0.1cm} \textit{#1:}}

\newcommand{\myminisection}[1]{\vspace{0.1cm} \noindent \textbf{#1.}}

\newcommand{\mysubsubsection}[1]{\subsubsection{\textbf{#1}}}

% \ifSPACEHACK
%     % Titlespacing args: \titlespacing{command}{left spacing}{before spacing}{after spacing}[right]
%     \titlespacing*\subsection{0pt}{2pt plus 1.5pt minus 1.5pt}{1pt plus 1.5pt minus 1.5pt}
%     \titlespacing*\subsubsection{0pt}{2pt plus 1pt minus 1pt}{2pt plus 1.5pt minus 1.5pt}
%     \titlespacing*\paragraph{0pt}{2.5pt plus 1.5pt minus 1.5pt}{2pt plus 1.5pt minus 1.5pt}
%     \setlength{\abovecaptionskip}{2pt plus 1pt minus 1pt}
%     \setlength{\belowcaptionskip}{2pt plus 1pt minus 1pt}
%     \setlength{\floatsep}{2.0pt plus 2.0pt minus 2.0pt}
%     %\setlength{\textfloatsep}{3.0pt plus 2.0pt minus 4.0pt}
%     %\setlength{\intextsep}{2.0pt plus 2.0pt minus 2.0pt}
% \fi

%%%%%%%%
% Peer review
%%%%%%%%


%%%%%%%%
% Balance references
%%%%%%%%

\usepackage{balance} % Put \balance on the last page
%\usepackage{caption}
%\usepackage[font=normal]{caption}
% \usepackage{subcaption}
%%%%
% Intra-paper references
%%%%

\usepackage{amsmath}
\usepackage{cleveref}


\crefformat{section}{\S#2#1#3}
\crefname{figure}{Figure}{Figures}
\crefname{appendix}{Appendix}{Appendices}
\crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{listing}{Listing}{Listings}
\crefname{theorem}{Theorem}{Theorems}
\crefname{thm}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{equation}{Eqt.}{Eqts.}
\crefformat{Grammar}{Grammar #1}


%%%%
% Tunable enumerate and itemize
%%%%

\usepackage{enumitem}
\usepackage{booktabs}

%%%%
% Latin
%%%%

\newcommand{\ie}{\textit{i.e.,} }
\newcommand{\eg}{\textit{e.g.,} }
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etals}{\textit{et al.'s}\xspace}
\newcommand{\nb}{\textit{N.B.,} }

\newcommand{\HF}{{Hugging Face}\xspace}
% Please add the following required packages to your document preamble:

\usepackage{enumitem}

%\usepackage{booktabs}
%\usepackage[normalem]{ulem}

% Nice formatting for a list of RQs
\newenvironment{RQList}{
   \setlength{\topsep}{0pt}
   \setlength{\partopsep}{0pt}
   \setlength{\parskip}{0pt}
   \begin{description}[style=unboxed]
   \setlength{\leftmargin}{1in}
   \setlength{\parsep}{0pt}
   \setlength{\parskip}{0pt}
   \setlength{\itemsep}{0pt}
   }
   {\end{description}}
   
\setlength{\abovecaptionskip}{2pt plus 1pt minus 1pt}
\setlength{\belowcaptionskip}{2pt plus 1pt minus 1pt}

\newcommand{\myquote}[1]{\begin{quote}\emph{``#1''}\end{quote}}
\newcommand{\myinlinequote}[1]{\emph{``#1''}}

\newcommand{\SmallLongString}[1]{ {\small \emph{#1}}\xspace}

% ParticipantID, Quote
\newcommand{\ParticipantQuote}[2]{
    \begin{quote}
    \emph{\textbf{#1}: ``#2''} 
    \end{quote}}
    
\DeclareUnicodeCharacter{2060}{\nolinebreak}

